Language Models can Evaluate Themselves via Probability Discrepancy

In this paper, we initiate our discussion by demonstrating how Large Language Models (LLMs), when tasked with responding to queries, display a more even probability distribution in their answers if they are more adept, as opposed to their less skilled counterparts. Expanding on this foundational insight, we propose a new self-evaluation method ProbDiff for assessing the efficacy of various LLMs. This approach obviates the necessity for an additional evaluation model or the dependence on external, proprietary models like GPT-4 for judgment. It uniquely utilizes the LLMs being tested to compute the probability discrepancy between the initial response and its revised versions. A higher discrepancy for a given query between two LLMs indicates a relatively weaker capability. Our findings reveal that ProbDiff achieves results on par with those obtained from evaluations based on GPT-4, spanning a range of scenarios that include natural language generation (NLG) tasks such as translation, summarization, and our proposed Xiaohongshu blog writing task, and benchmarks for LLM evaluation like AlignBench, MT-Bench, and AlpacaEval, across LLMs of varying magnitudes.

==> tex/table-example.tex <==


\begin{table*}[t]
\renewcommand\arraystretch{1.1} 
\renewcommand\tabcolsep{4pt}
	\centering
	\begin{tabular}{l|l|cccccccccccc}
	\toprule
	\multicolumn{2}{c|}{\multirow{2}{*}{}} 
	&\multicolumn{2}{c}{\textbf{Cs-En}} 
	&\multicolumn{2}{c}{\textbf{De-En}}
        &\multicolumn{2}{c}{\textbf{Ru-En}} 
	&\multicolumn{2}{c}{\textbf{Zh-En}}
        &\multicolumn{2}{c}{\textbf{Xsum}}
        &\multicolumn{2}{c}{\textbf{Cnn\_dm}}\\
	\multicolumn{2}{c|}{} &Base &FT &Base &FT &Base&FT &Base&FT &Base&FT &Base &FT \\
	\midrule
    %\multicolumn{10}{l}{\textbf{Dataless}}\\

\multirow{2}{*}{\textbf{turn 1}} & inc & 34.8 & 53.8 & 22.2 & 53.8 & 73.4 &\underline{21.7} & 76.0 & \\

\multirow{2}{*}{} & eq & 34.8 & 53.8 & 22.2 & 53.8 & 73.4 &\underline{21.7} & 76.0 & \\
	
\bottomrule
\end{tabular}
\caption{example} 
\label{tab:perf}
\end{table*}


